Pareto-Conditioned Diffusion Models for Offline Multi-Objective Optimization

Multi-objective optimization (MOO) arises in many real-world applications where trade-offs between competing objectives must be carefully balanced. In the offline setting, where only a static dataset is available, the main challenge is generalizing beyond observed data. We introduce Pareto-Conditioned Diffusion (PCD), a novel framework that formulates offline MOO as a conditional sampling problem. By conditioning directly on desired trade-offs, PCD avoids the need for explicit surrogate models. To effectively explore the Pareto front, PCD employs a reweighting strategy that focuses on high-performing samples and a reference-direction mechanism to guide sampling towards novel, promising regions beyond the training data. Experiments on standard offline MOO benchmarks show that PCD achieves highly competitive performance and, importantly, demonstrates greater consistency across diverse tasks than existing offline MOO approaches.

==> result_tables/ablation_18-09-25.tex <==
\begin{tabular}{lrrrr}
\toprule
\textbf{Method} & C10/MOP2 & MO-Swimmer-v2 & RE34 & ZDT2 \\
\midrule
w/o ref-dir \& w/o pre-processing & 10.46 & 1.76 & 9.19 & \underline 7.59 \\
w pruning & 10.55 & \underline 3.63 & \underline 10.16 & 5.64 \\
w/o preprocessing & 10.47 & 3.53 & 10.11 & \bfseries 7.89 \\
w/o ref-dir & \underline 10.57 & 1.85 & 9.44 & 6.34 \\
\midrule
PC-Diffusion & \bfseries 10.59 & \bfseries 3.69 & \bfseries 10.17 & 6.25 \\
\bottomrule
\end{tabular}


==> result_tables/ablation_19-09-25.tex <==
\begin{tabular}{lrrrr}
\toprule
\textbf{Method} & C10/MOP2 & MO-Swimmer-v2 & RE34 & ZDT2 \\
\midrule
baseline & 10.46 & 1.76 & 9.19 & \underline {7.59} \\
w pruning & 10.55 & \underline{3.63} & \underline {10.16} & 5.64 \\
w/o preprocessing & 10.47 & 3.53 & 10.11 & \bfseries 7.89 \\
w/o ref-dir & \underline{10.57} & 1.85 & 9.44 & 6.34 \\
\midrule
PC-Diffusion & \bfseries 10.59 & \bfseries 3.69 & \bfseries 10.17 & 6.25 \\
\bottomrule
\end{tabular}


==> result_tables/ablation_table.tex <==
\begin{tabular}{lccccc}
\toprule
\textbf{Variant} & ZDT2 & MO-Swimmer-v2 & RE34 & Regex & C10/MOP2 \\
\midrule
Ideal + N/A & \underline{7.59$\pm$0.19} & 1.76$\pm$0.21 & 9.19$\pm$0.26 & \textbf{5.60$\pm$0.35} & 10.46$\pm$0.01 \\
Ref. Dir. + N/A& \textbf{7.89$\pm$0.19} & 3.53$\pm$0.11 & 10.11$\pm$0.03 & \underline{5.55$\pm$0.25} & 10.47$\pm$0.01 \\
Ref. Dir. + Pruning & 5.64$\pm$0.13 & \underline{3.63$\pm$0.07} & \underline{10.16$\pm$0.03} & 4.20$\pm$0.64 & \underline{10.55$\pm$0.08} \\
\midrule
PCD & 6.25$\pm$0.06 & \textbf{3.69$\pm$0.11} & \textbf{10.17$\pm$0.04} & 4.80$\pm$0.87 & \textbf{10.59$\pm$0.04} \\
\bottomrule
\end{tabular}


==> result_tables/ablation_table_t.tex <==
\begin{tabular}{l|cccc}
\toprule
\textbf{Task} & Ideal + N/A & Ref. Dir + N/A & Ref.Dir + Pruning & PCD \\
\midrule
C10/MOP2 & 10.46$\pm$0.01 & 10.47$\pm$0.01 & 10.55$\pm$0.08 &  \textbf{10.59$\pm$0.04} \\
MO-Swimmer-v2 & 1.76$\pm$0.21 & 3.53$\pm$0.11 & \underline{3.63$\pm$0.07} & \textbf{3.69$\pm$0.11} \\
RE34 & 9.19$\pm$0.26 & 10.11$\pm$0.03 & \underline{10.16$\pm$0.03}  & \textbf{10.17$\pm$0.04} \\
Regex & \textbf{5.60$\pm$0.35} & \underline{5.55$\pm$0.25} & 4.20$\pm$0.64 &  4.80$\pm$0.87 \\
ZDT2 & \underline{7.59$\pm$0.19} & \textbf{7.89$\pm$0.19} & 5.64$\pm$0.13 & 6.25$\pm$0.06 \\
\bottomrule
\end{tabular}


==> result_tables/main_table.tex <==
\begin{tabular}{lcccccc}
\toprule
\textbf{Method} & Synthetic & MORL & RE & Scientific & MONAS & Avg. rank \\
\midrule
$\mathcal{D}$(best) & 5.45$\pm$0.19 & \textbf{1.70$\pm$0.27} & 2.60$\pm$0.07 & 9.10$\pm$0.14 & 11.53$\pm$0.06 & 7.41$\pm$0.05 \\
End2End + GN & 7.33$\pm$0.55 & 5.70$\pm$2.14 & 7.06$\pm$0.32 & 5.25$\pm$1.27 & 9.33$\pm$0.53 & 7.81$\pm$0.39 \\
End2End + PC & 5.93$\pm$0.25 & \underline{3.50$\pm$1.22} & 6.22$\pm$0.33 & 4.15$\pm$1.33 & 6.60$\pm$0.40 & 6.00$\pm$0.29 \\
End2End & 6.16$\pm$0.30 & 9.70$\pm$2.08 & 6.06$\pm$0.30 & 4.15$\pm$1.39 & \underline{5.13$\pm$0.22} & \underline{5.71$\pm$0.15} \\
MOBO & 8.69$\pm$0.30 & 14.60$\pm$0.42 & 10.00$\pm$0.33 & 6.55$\pm$0.48 & 8.11$\pm$0.80 & 8.80$\pm$0.35 \\
MultiHead + GN & 8.82$\pm$0.53 & 8.90$\pm$2.16 & 8.14$\pm$0.94 & 5.00$\pm$2.05 & 12.57$\pm$0.40 & 9.83$\pm$0.32 \\
MultiHead + PC & 8.87$\pm$0.45 & 10.90$\pm$1.08 & 6.74$\pm$0.68 & 6.00$\pm$0.85 & 7.46$\pm$0.30 & 7.67$\pm$0.32 \\
MultiHead & 6.18$\pm$0.53 & 8.00$\pm$1.41 & 6.14$\pm$0.29 & 5.55$\pm$0.89 & 5.88$\pm$0.49 & 6.08$\pm$0.22 \\
MM + COM & 8.02$\pm$0.47 & 3.60$\pm$1.29 & 6.54$\pm$0.17 & \underline{3.70$\pm$0.57} & 7.22$\pm$0.43 & 6.79$\pm$0.12 \\
MM + ICT & 6.73$\pm$0.46 & 9.10$\pm$1.95 & 5.44$\pm$0.32 & 4.95$\pm$0.65 & 8.42$\pm$0.40 & 7.07$\pm$0.13 \\
MM + IOM & 5.16$\pm$0.51 & 12.70$\pm$0.91 & 5.76$\pm$0.52 & 4.25$\pm$1.09 & 5.77$\pm$0.50 & 5.79$\pm$0.19 \\
MM + TM & 6.55$\pm$0.82 & 7.90$\pm$2.16 & 5.78$\pm$0.25 & 5.80$\pm$1.16 & 7.87$\pm$0.39 & 6.90$\pm$0.19 \\
MM & 6.07$\pm$0.50 & 9.50$\pm$0.79 & 5.94$\pm$0.41 & 6.35$\pm$0.82 & \textbf{4.97$\pm$0.46} & 5.78$\pm$0.20 \\
ParetoFlow & \textbf{2.44$\pm$0.28} & 8.50$\pm$1.32 & \underline{1.74$\pm$0.17} & 8.80$\pm$0.27 & 11.19$\pm$0.52 & 6.71$\pm$0.23 \\
\midrule
PCD & \underline{3.38$\pm$0.20} & 5.50$\pm$3.30 & \textbf{1.51$\pm$0.13} & \textbf{3.27$\pm$1.01} & 7.54$\pm$0.50 & \textbf{4.76$\pm$0.30} \\
\bottomrule
\end{tabular}


==> result_tables/morl_hv_100th.tex <==
\begin{tabular}{lcc}
\toprule
\textbf{Method} & MO-Hopper-v2 & MO-Swimmer-v2 \\
\midrule
$\mathcal{D}$(best) & \textbf{6.33$\pm$0.00} & \textbf{3.70$\pm$0.00} \\
E2E + GN & 5.94$\pm$0.33 & 3.65$\pm$0.02 \\
E2E + PC & \underline{6.22$\pm$0.15} & 3.66$\pm$0.00 \\
E2E & 5.98$\pm$0.34 & 1.68$\pm$0.75 \\
MOBO & 4.75$\pm$0.00 & 0.86$\pm$0.00 \\
MH + GN & 5.73$\pm$0.26 & 3.49$\pm$0.16 \\
MH + PC & 4.99$\pm$0.34 & 3.42$\pm$0.36 \\
MH & 5.64$\pm$0.54 & 3.20$\pm$0.98 \\
MM + COM & 6.14$\pm$0.15 & 3.68$\pm$0.02 \\
MM + ICT & 5.67$\pm$0.26 & 3.12$\pm$1.11 \\
MM + IOM & 4.95$\pm$0.44 & 1.95$\pm$0.53 \\
MM + TM & 5.93$\pm$0.30 & 3.55$\pm$0.05 \\
MM & 5.99$\pm$0.19 & 1.61$\pm$0.58 \\
ParetoFlow & 5.92$\pm$0.05 & 3.50$\pm$0.10 \\
\midrule
PCD (ours) & 5.95$\pm$0.18 & \underline{3.69$\pm$0.11} \\
\bottomrule
\end{tabular}


==> result_tables/re_hv_100th.tex <==
\begin{tabular}{lccccccccccccccc}
\toprule
\textbf{Method} & RE21 & RE22 & RE23 & RE24 & RE25 & RE31 & RE32 & RE33 & RE34 & RE35 & RE36 & RE37 & RE41 & RE42 & RE61 \\
\midrule
$\mathcal{D}$(best) & \underline{4.10$\pm$0.00} & 4.78$\pm$0.00 & 4.75$\pm$0.00 & 4.60$\pm$0.00 & 4.79$\pm$0.00 & \underline{10.60$\pm$0.00} & 10.56$\pm$0.00 & 10.56$\pm$0.00 & 9.30$\pm$0.00 & 10.08$\pm$0.00 & 7.61$\pm$0.00 & 5.57$\pm$0.00 & \textbf{18.27$\pm$0.00} & 14.52$\pm$0.00 & 97.49$\pm$0.00 \\
E2E + GN & 2.60$\pm$0.00 & 3.18$\pm$0.00 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.81$\pm$0.17 & 5.06$\pm$0.73 & 4.96$\pm$0.13 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.13$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
E2E + PC & 2.60$\pm$0.00 & 1.91$\pm$1.74 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.29$\pm$0.71 & 6.54$\pm$0.13 & 7.07$\pm$0.32 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.12$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
E2E & 2.60$\pm$0.00 & 3.18$\pm$0.00 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.93$\pm$0.07 & 6.62$\pm$0.00 & 7.14$\pm$0.20 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.12$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MOBO & 1.98$\pm$0.02 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 4.02$\pm$0.04 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 2.80$\pm$0.00 & 13.03$\pm$0.03 & 0.00$\pm$0.00 & \underline{nan} \\
MH + GN & 2.58$\pm$0.03 & 1.91$\pm$1.74 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.19$\pm$0.61 & 5.97$\pm$0.36 & 4.37$\pm$0.73 & 0.00$\pm$0.00 & 5.89$\pm$0.38 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.33$\pm$0.00 & 14.99$\pm$0.12 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MH + PC & 2.60$\pm$0.00 & 1.91$\pm$1.74 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 6.42$\pm$0.46 & 5.54$\pm$3.16 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.12$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MH & 2.60$\pm$0.00 & 3.18$\pm$0.00 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.41$\pm$0.73 & 6.62$\pm$0.00 & 7.28$\pm$0.00 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.12$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MM + COM & 2.59$\pm$0.00 & 1.64$\pm$1.60 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.98$\pm$0.00 & 5.67$\pm$1.56 & 7.28$\pm$0.00 & 0.00$\pm$0.00 & 6.31$\pm$0.01 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.33$\pm$0.00 & 15.10$\pm$0.04 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MM + ICT & 2.60$\pm$0.00 & 3.18$\pm$0.00 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.98$\pm$0.00 & 6.54$\pm$0.08 & 7.28$\pm$0.00 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.13$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MM + IOM & 2.60$\pm$0.00 & 3.18$\pm$0.00 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.93$\pm$0.07 & 6.62$\pm$0.00 & 7.28$\pm$0.00 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.13$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MM + TM & 2.60$\pm$0.00 & 3.18$\pm$0.00 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.27$\pm$0.64 & 6.62$\pm$0.00 & 7.28$\pm$0.00 & 0.00$\pm$0.00 & 6.31$\pm$0.01 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.12$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
MM & 2.60$\pm$0.00 & 3.18$\pm$0.00 & 0.00$\pm$0.00 & 1.66$\pm$0.00 & 3.77$\pm$0.08 & 6.62$\pm$0.00 & 7.28$\pm$0.00 & 0.00$\pm$0.00 & 6.31$\pm$0.00 & 0.00$\pm$0.00 & 0.00$\pm$0.00 & 3.34$\pm$0.00 & 15.12$\pm$0.00 & 0.00$\pm$0.00 & 45.11$\pm$0.00 \\
ParetoFlow & 4.09$\pm$0.06 & \underline{4.78$\pm$0.07} & \underline{4.80$\pm$0.02} & \textbf{5.04$\pm$0.06} & \underline{4.96$\pm$0.15} & 10.56$\pm$0.14 & \underline{11.03$\pm$0.38} & \underline{10.84$\pm$0.24} & \textbf{11.69$\pm$1.33} & \textbf{11.12$\pm$0.43} & \textbf{8.67$\pm$0.17} & \textbf{6.51$\pm$0.58} & \underline{18.20$\pm$0.41} & \textbf{54.44$\pm$22.78} & \textbf{112.08$\pm$11.62} \\
PCD (ours) & \textbf{4.35$\pm$0.00} & \textbf{4.89$\pm$0.01} & \textbf{4.84$\pm$0.00} & \underline{4.88$\pm$0.02} & \textbf{5.06$\pm$0.03} & \textbf{11.35$\pm$0.06} & \textbf{19.94$\pm$5.75} & \textbf{10.97$\pm$0.09} & \underline{10.17$\pm$0.04} & \underline{10.87$\pm$0.04} & \underline{8.16$\pm$0.11} & \underline{5.97$\pm$0.01} & 18.14$\pm$0.02 & \underline{15.49$\pm$0.03} & nan \\
\bottomrule
\end{tabular}


==> result_tables/synthetic_hv_100th.tex <==
\begin{tabular}{lccccccccccc}
\toprule
 & \multicolumn{11}{r}{value} \\
task & DTLZ1 & DTLZ7 & OMNITEST & VLMOP1 & VLMOP2 & VLMOP3 & ZDT1 & ZDT2 & ZDT3 & ZDT4 & ZDT6 \\
method &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
$\mathcal{D}$(best) & 10.60$\pm$0.00 & 8.56$\pm$0.00 & 4.53$\pm$0.00 & \textbf{\underline{0.41$\pm$0.00}} & 1.78$\pm$0.00 & 45.65$\pm$0.00 & \underline{4.17$\pm$0.00} & 4.68$\pm$0.00 & 5.15$\pm$0.00 & \textbf{5.46$\pm$0.00} & \textbf{4.61$\pm$0.00} \\
E2E + GN & 10.63$\pm$0.00 & 8.95$\pm$0.00 & 4.55$\pm$0.14 & 0.29$\pm$0.00 & 2.80$\pm$0.16 & 41.93$\pm$1.13 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.75$\pm$0.00 & 4.87$\pm$0.05 & 3.82$\pm$0.03 \\
E2E + PC & 10.63$\pm$0.00 & 8.95$\pm$0.00 & 4.69$\pm$0.06 & 0.29$\pm$0.00 & 3.34$\pm$0.01 & 42.45$\pm$0.00 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.75$\pm$0.00 & 4.84$\pm$0.09 & 3.78$\pm$0.08 \\
E2E & 10.61$\pm$0.01 & 8.95$\pm$0.00 & 4.69$\pm$0.05 & 0.29$\pm$0.00 & \underline{3.36$\pm$0.00} & 42.45$\pm$0.00 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.76$\pm$0.00 & 4.82$\pm$0.02 & 3.83$\pm$0.01 \\
MOBO & 10.40$\pm$0.06 & 3.96$\pm$0.10 & \underline{4.76$\pm$0.01} & 0.29$\pm$0.00 & 2.08$\pm$0.16 & 38.99$\pm$0.14 & 2.38$\pm$0.01 & 2.76$\pm$0.00 & 3.13$\pm$0.05 & 4.93$\pm$0.09 & 3.76$\pm$0.00 \\
MH + GN & 10.63$\pm$0.01 & 8.95$\pm$0.00 & 4.61$\pm$0.09 & 0.08$\pm$0.03 & 3.15$\pm$0.07 & 30.14$\pm$6.91 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.76$\pm$0.00 & 4.83$\pm$0.05 & 3.74$\pm$0.04 \\
MH + PC & 10.63$\pm$0.00 & 8.95$\pm$0.00 & 4.48$\pm$0.22 & 0.20$\pm$0.04 & 2.98$\pm$0.09 & 41.85$\pm$0.91 & 2.41$\pm$0.27 & 2.68$\pm$0.01 & 3.68$\pm$0.16 & 4.83$\pm$0.04 & 3.76$\pm$0.04 \\
MH & 10.63$\pm$0.00 & 8.95$\pm$0.00 & 4.61$\pm$0.09 & 0.29$\pm$0.00 & 3.32$\pm$0.01 & 42.45$\pm$0.00 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.76$\pm$0.00 & 4.87$\pm$0.02 & 3.83$\pm$0.01 \\
MM + COM & 10.62$\pm$0.00 & 8.95$\pm$0.00 & 4.54$\pm$0.15 & 0.23$\pm$0.13 & 1.68$\pm$0.04 & 42.44$\pm$0.02 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.75$\pm$0.00 & 4.84$\pm$0.03 & 3.82$\pm$0.04 \\
MM + ICT & 10.63$\pm$0.00 & 8.95$\pm$0.00 & 4.56$\pm$0.08 & 0.29$\pm$0.00 & 3.35$\pm$0.01 & 42.43$\pm$0.01 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.76$\pm$0.00 & 4.86$\pm$0.04 & 3.83$\pm$0.02 \\
MM + IOM & 10.63$\pm$0.00 & 8.95$\pm$0.00 & 4.72$\pm$0.03 & 0.29$\pm$0.00 & 3.32$\pm$0.03 & 42.45$\pm$0.01 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.73$\pm$0.05 & 4.85$\pm$0.03 & 3.84$\pm$0.01 \\
MM + TM & 10.63$\pm$0.00 & 8.95$\pm$0.01 & 4.59$\pm$0.10 & 0.29$\pm$0.00 & 3.35$\pm$0.00 & 42.41$\pm$0.01 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.73$\pm$0.05 & 4.80$\pm$0.10 & 3.84$\pm$0.00 \\
MM & 10.63$\pm$0.00 & 8.95$\pm$0.00 & 4.71$\pm$0.06 & 0.29$\pm$0.00 & 3.35$\pm$0.01 & 42.45$\pm$0.00 & 2.81$\pm$0.00 & 3.17$\pm$0.00 & 3.76$\pm$0.00 & 4.85$\pm$0.06 & 3.82$\pm$0.00 \\
ParetoFlow & \underline{11.15$\pm$0.44} & \underline{10.54$\pm$0.44} & \textbf{4.78$\pm$0.00} & nan & \textbf{4.22$\pm$0.02} & \textbf{45.92$\pm$0.00} & 4.15$\pm$0.04 & \underline{5.71$\pm$0.21} & \underline{5.22$\pm$0.11} & 4.86$\pm$0.08 & 4.51$\pm$0.05 \\
PCD (ours) & \textbf{13.63$\pm$0.78} & \textbf{11.35$\pm$0.18} & 4.76$\pm$0.01 & 0.09$\pm$0.01 & 2.93$\pm$0.28 & \underline{45.91$\pm$0.01} & \textbf{4.47$\pm$0.02} & \textbf{6.25$\pm$0.06} & \textbf{5.36$\pm$0.36} & \underline{5.23$\pm$0.06} & \underline{4.56$\pm$0.05} \\
\bottomrule
\end{tabular}

